World-Ego Modeling for Embodied Video Generation in Long-Horizon Navigation-Manipulation Tasks

Embodied video world models typically capture both scene evolution and the robot's behavior, which we refer to as the \emph{world} and the \emph{ego}, respectively. The world and the ego exhibit different underlying dynamics: world prediction relies primarily on visual history and emphasizes scene stability, whereas ego prediction relies more strongly on the current instruction and emphasizes accurate instruction following. Modeling both components within a single generation stream can entangle these different dependencies, making it difficult to specialize the prediction of either component. Consequently, it becomes difficult to simultaneously maintain scene consistency and accurate instruction following, particularly in long-horizon navigation-manipulation tasks. In this paper, we propose to decompose an embodied video into the world and the ego and disentangle their generation processes. Specifically, we define the world as the background and currently unmanipulated objects, and the ego as the robot and currently manipulated objects. Based on this definition, we develop the \emph{World-Ego Model} (WEM), which combines a vision-language state predictor using role-conditioned attention (RCA) and asymmetric query budgets with a semantic-routed mixture-of-experts (SR-MoE) diffusion generator. To enable rigorous evaluation, we further construct HTEWorld, a dataset and benchmark for long-horizon embodied video generation with hybrid navigation-manipulation tasks, providing 125K training video clips comprising over 4.5M frames with fine-grained instructions, together with 300 multi-turn evaluation trajectories covering over 2K instructions. Extensive experiments show that WEM achieves state-of-the-art performance on HTEWorld while remaining competitive on existing manipulation-oriented evaluations.

==> Figures/fig_example.tex <==
\begin{figure}[!t]
  \begin{center}
    \includegraphics[width=\linewidth]{Images/teaser.jpg}
  \end{center}
  \caption{\small Figure caption.}
  \label{fig:label}
\end{figure}

==> Figures/views.tex <==
\begin{figure}[t!]
\begin{center}
% \vspace{-0.3cm}
\includegraphics[width=0.95\linewidth]{Images/fig7_views.pdf}
% \vspace{-0.1cm}
\caption{
Three perspectives of the world-ego definition.
The motion-based view separates the world and ego by the source of visual motion; the semantic-based view separates them by the embodied role of scene entities; and the intention-based view separates them by the source of conditioning information.
We adopt the semantic-based view as the default world-ego definition in WEM.
}
\label{fig:views}
\end{center}
\vspace{-0.3cm}
\end{figure}

==> Tables/tab_design_studies.tex <==
\begin{table}[t]
\centering
\begin{minipage}[t]{0.43\linewidth}
\centering
\small
\setlength{\tabcolsep}{5pt}
\caption{\small Design study on world-ego definitions. We report EWMScore on HTEWorld.} 
%under the WorldArena protocol.}
\label{tab:boundary_study}
\begin{tabular}{lc}
\toprule
World-ego definition & EWMScore \\
\midrule
Intention-based view & 58.69 \\
Motion-based view & 59.36 \\
Semantic-based view & \textbf{61.48} \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.54\linewidth}
\centering
\small
\setlength{\tabcolsep}{4pt}
\caption{\small Design study on world-ego disentanglement strategies. All variants use the semantic-based view.}
\label{tab:disentanglement_study}
\begin{tabular}{lc}
\toprule
Variant & EWMScore \\
\midrule
w/o Disent. & 58.40 \\
Pre-Disent. & 58.85 \\
Post-Disent. w/o or w/ Semantic Proxy & 58.59/61.09\\
% Post-Disent. &  \\
Full Disent. (WEM) & \textbf{61.48} \\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-2mm}
\end{table}

==> Tables/tab_example.tex <==
\begin{table}[!t]
  \caption{Sample table title}
  \centering
  \begin{tabular}{lll}
    \toprule
    Name & Description & Size ($\mu$m) \\
    \midrule
    Dendrite & Input terminal & $\sim$100 \\
    Axon & Output terminal & $\sim$10 \\
    Soma & Cell body & up to $10^6$ \\
    \bottomrule
  \end{tabular}
  \label{tab:table}
\end{table}

==> Tables/tab_specific_and_worldarena.tex <==
% \begin{table*}[t]
% \centering
% \small
% \begin{minipage}[t]{0.54\textwidth}
% \centering
% \scriptsize
% \setlength{\tabcolsep}{2pt}
% \caption{\small Comparison on HTEWorld w/ navigation-manipulation metrics. All scores are reported in their original scale, and higher is better.}
% \label{tab:hteworld_specific_metrics}
% \begin{tabular}{lcccccc}
% \toprule
% Model & RCBD & LPSA & CISR & PMPA & CPDM & FPHS \\
% \midrule
% WoW-7B~\citep{bib:wow}        & 0.23 & 0.83 & 0.49 & 0.45 & 0.47 & 0.85 \\
% Cosmos-2B~\citep{bib:cosmos_predict}     & 0.24 & 0.83 & 0.50 & 0.47 & 0.48 & 0.86 \\
% Cosmos-14B~\citep{bib:cosmos_predict}    & 0.26 & 0.83 & 0.51 & 0.48 & 0.49 & 0.85 \\
% PAN-style~\citep{bib:pan}     & 0.27 & 0.86 & 0.49 & 0.50 & 0.46 & 0.88 \\
% \midrule
% Intention-based view & 0.28 & 0.86 & 0.53 & 0.52 & 0.50 & 0.88 \\
% Motion-based view & 0.29 & 0.87 & 0.53 & 0.54 & 0.51 & 0.89 \\
% \rowcolor[HTML]{D9E1F2} WEM           & \textbf{0.31} & \textbf{0.87} & \textbf{0.57} & \textbf{0.54} & \textbf{0.52} & \textbf{0.89} \\
% \bottomrule
% \end{tabular}
% \end{minipage}
% \hfill
% \begin{minipage}[t]{0.42\textwidth}
% \centering
% \small
% \setlength{\tabcolsep}{7pt}
% \caption{\small Comparison on WorldArena. Related scores were reported in WorldArena paper; WEM is evaluated with the same protocol.}
% \label{tab:original_worldarena}
% \begin{tabular}{lc}
% \toprule
% Model & EWMScore \\
% \midrule
% Wan2.2~\citep{bib:wan} & 54.54 \\
% WoW~\citep{bib:wow} & 54.88 \\
% Cosmos-Predict 2.5 (Action)~\citep{bib:cosmos_predict} & 55.91 \\
% CogVideoX~\citep{bib:cogvideox} & 57.90 \\
% \rowcolor[HTML]{D9E1F2} WEM (ours) & 58.10 \\
% IRASim~\citep{bib:irasim} & 58.12 \\
% CtrlWorld~\citep{bib:ctrl_world} & \textbf{59.70} \\
% \bottomrule
% \end{tabular}
% \vspace{1mm}
% % {\footnotesize $^\dagger$ denotes our model.}
% \end{minipage}
% \vspace{-2mm}
% \end{table*}

\begin{table*}[!t]
\centering
\vspace{-0.2cm}
\begin{minipage}[t]{0.55\textwidth}
\centering
\caption{\small Comparison on HTEWorld w/ navigation-manipulation metrics. Scores are reported in their original scale, and higher is better.}
\label{tab:hteworld_specific_metrics}
\vspace{-0.15cm}
\scriptsize
\setlength{\tabcolsep}{2pt}
\begin{tabular}{lcccccc}
\toprule
Model & RCBD & LPSA & CISR & PMPA & CPDM & FPHS \\
\midrule
WoW-7B~\citep{bib:wow}        & 0.23 & 0.83 & 0.49 & 0.45 & 0.47 & 0.85 \\
Cosmos-2B~\citep{bib:cosmos_predict}     & 0.24 & 0.83 & 0.50 & 0.47 & 0.48 & 0.86 \\
Cosmos-14B~\citep{bib:cosmos_predict}    & 0.26 & 0.83 & 0.51 & 0.48 & 0.49 & 0.85 \\
PAN-style~\citep{bib:pan}     & 0.27 & 0.86 & 0.49 & 0.50 & 0.46 & 0.88 \\
\midrule
Intention-based & 0.28 & 0.86 & 0.53 & 0.52 & 0.50 & 0.88 \\
Motion-based & 0.29 & \textbf{0.87} & 0.53 & \textbf{0.54} & 0.51 & \textbf{0.89} \\
\rowcolor[HTML]{D9E1F2} WEM
& \textbf{0.31} & \textbf{0.87} & \textbf{0.57} & \textbf{0.54} & \textbf{0.52} & \textbf{0.89} \\
\bottomrule
\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.41\textwidth}
\centering
\caption{\small Comparison on WorldArena. Related scores are from the WorldArena paper; WEM uses the same protocol.}
\label{tab:original_worldarena}
\vspace{-0.15cm}
\scriptsize
\setlength{\tabcolsep}{5pt}
\begin{tabular}{lc}
\toprule
Model & EWMScore \\
\midrule
Wan2.2~\citep{bib:wan} & 54.54 \\
WoW~\citep{bib:wow} & 54.88 \\
Cosmos-Predict 2.5 (Action)~\citep{bib:cosmos_predict} & 55.91 \\
CogVideoX~\citep{bib:cogvideox} & 57.90 \\
\rowcolor[HTML]{D9E1F2} WEM (ours) & 58.10 \\
IRASim~\citep{bib:irasim} & 58.12 \\
CtrlWorld~\citep{bib:ctrl_world} & \textbf{59.70} \\
\bottomrule
\end{tabular}
\end{minipage}
\vspace{-0.25cm}
\end{table*}

==> Tables/tab_wem_ablation.tex <==
\begin{table}[h]
\centering
\small
\setlength{\tabcolsep}{6pt}
\caption{Component ablation of WEM on HTEWorld under the WorldArena evaluation protocol. Higher is better.}
\label{tab:wem_ablation}
\begin{tabular}{lc}
\toprule
Variant & EWMScore \\
\midrule
w/o Asymmetric Query Budget & 60.50 \\
w/o Role-Conditioned Attention & 60.64 \\
w/o Neighbor-Expanded Routing & 59.57 \\
\midrule
WEM & \textbf{61.48} \\
\bottomrule
\end{tabular}
\end{table}

